The Ink Splotch Effect: A Case Study on ChatGPT as a Co-Creative Game Designer

This paper studies how large language models (LLMs) can act as effective, high-level creative collaborators and ``muses'' for game design. We model the design of this study after the exercises artists use by looking at amorphous ink splotches for creative inspiration. Our goal is to determine whether AI-assistance can improve, hinder, or provide an alternative quality to games when compared to the creative intents implemented by human designers. The capabilities of LLMs as game designers are stress tested by placing it at the forefront of the decision making process. Three prototype games are designed across 3 different genres: (1) a minimalist base game, (2) a game with features and game feel elements added by a human game designer, and (3) a game with features and feel elements directly implemented from prompted outputs of the LLM, ChatGPT. A user study was conducted and participants were asked to blindly evaluate the quality and their preference of these games. We discuss both the development process of communicating creative intent to an AI chatbot and the synthesized open feedback of the participants. We use this data to determine both the benefits and shortcomings of AI in a more design-centric role.

==> ext_tex/color_rank_table_mini.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{l|ccc|ccc|ccc|}
\cline{2-10}
 &
  \multicolumn{3}{c|}{\cellcolor[HTML]{CBCEFB}Space Shooter} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{FFCE93}Platformer} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{C0C0C0}Roguelike} \\ \cline{2-10} 
 &
  \multicolumn{1}{l}{$S_{H}$} &
  \multicolumn{1}{l}{$S_{C}$} &
  \multicolumn{1}{l|}{$S_{B}$} &
  \multicolumn{1}{l}{$S_{H}$} &
  \multicolumn{1}{l}{$S_{C}$} &
  \multicolumn{1}{l|}{$S_{B}$} &
  \multicolumn{1}{l}{$S_{H}$} &
  \multicolumn{1}{l}{$S_{C}$} &
  \multicolumn{1}{l|}{$S_{B}$} \\ \hline
\multicolumn{1}{|l|}{$C_{1}$} &
  \cellcolor[HTML]{CCEDCC}110 &
  \cellcolor[HTML]{FAF8C4}88 &
  \cellcolor[HTML]{E4A9A9}48 &
  \cellcolor[HTML]{CCEDCC}97 &
  \cellcolor[HTML]{FAF8C4}77 &
  \cellcolor[HTML]{E4A9A9}57 &
  \cellcolor[HTML]{CCEDCC}87 &
  \cellcolor[HTML]{FAF8C4}77 &
  \cellcolor[HTML]{E4A9A9}64 \\
\multicolumn{1}{|l|}{$C_{2}$} &
  \cellcolor[HTML]{CCEDCC}108 &
  \cellcolor[HTML]{FAF8C4}85 &
  \cellcolor[HTML]{E4A9A9}48 &
  \cellcolor[HTML]{CCEDCC}86 &
  \cellcolor[HTML]{E4A9A9}73 &
  \cellcolor[HTML]{FAF8C4}75 &
  \cellcolor[HTML]{CCEDCC}92 &
  \cellcolor[HTML]{FAF8C4}71 &
  \cellcolor[HTML]{E4A9A9}65 \\
\multicolumn{1}{|l|}{$C_{3}$} &
  \cellcolor[HTML]{FAF8C4}93 &
  \cellcolor[HTML]{CCEDCC}95 &
  \cellcolor[HTML]{E4A9A9}49 &
  \cellcolor[HTML]{CCEDCC}104 &
  \cellcolor[HTML]{FAF8C4}76 &
  \cellcolor[HTML]{E4A9A9}48 &
  \cellcolor[HTML]{CCEDCC}93 &
  \cellcolor[HTML]{FAF8C4}65 &
  \cellcolor[HTML]{E4A9A9}52 \\
\multicolumn{1}{|l|}{$C_{4}$} &
  \cellcolor[HTML]{CCEDCC}91 &
  \cellcolor[HTML]{FAF8C4}80 &
  \cellcolor[HTML]{E4A9A9}63 &
  \cellcolor[HTML]{CCEDCC}98 &
  \cellcolor[HTML]{FAF8C4}66 &
  \cellcolor[HTML]{E4A9A9}58 &
  \cellcolor[HTML]{CCEDCC}79 &
  \cellcolor[HTML]{FAF8C4}66 &
  \cellcolor[HTML]{E4A9A9}65 \\
\multicolumn{1}{|l|}{$C_{5}$} &
  \cellcolor[HTML]{CCEDCC}101 &
  \cellcolor[HTML]{FAF8C4}92 &
  \cellcolor[HTML]{E4A9A9}47 &
  \cellcolor[HTML]{CCEDCC}103 &
  \cellcolor[HTML]{FAF8C4}85 &
  \cellcolor[HTML]{E4A9A9}46 &
  \cellcolor[HTML]{CCEDCC}96 &
  \cellcolor[HTML]{FAF8C4}65 &
  \cellcolor[HTML]{E4A9A9}55 \\
\multicolumn{1}{|l|}{$C_{6}$} &
  \cellcolor[HTML]{CCEDCC}107 &
  \cellcolor[HTML]{FAF8C4}83 &
  \cellcolor[HTML]{E4A9A9}50 &
  \cellcolor[HTML]{CCEDCC}98 &
  \cellcolor[HTML]{E4A9A9}56 &
  \cellcolor[HTML]{FAF8C4}68 &
  \cellcolor[HTML]{CCEDCC}83 &
  \cellcolor[HTML]{FAF8C4}75 &
  \cellcolor[HTML]{E4A9A9}58 \\ \hline
\end{tabular}
\caption{\textbf{Scores for each game and genre using the formula $S_{G}$ and category criteria $C_{\#}$} Models with the highest score are colored in green, second highest in yellow, and lowest in red.}
\label{tab:score-table}
\end{table}
\vspace{10px}

==> ext_tex/grey_rank_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\begin{tabular}{l|lll|lll|lll|}
\cline{2-10}
 &
  \multicolumn{3}{c|}{\cellcolor[HTML]{CBCEFB}Space Shooter (\%)} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{AAE4A9}Platformer (\%)} &
  \multicolumn{3}{c|}{\cellcolor[HTML]{c0c0c0}Roguelike (\%)} \\ \cline{2-10} 
 &
  Human &
  ChatGPT &
  Base &
  Human &
  ChatGPT &
  Base &
  Human &
  ChatGPT &
  Base \\ \hline
\multicolumn{1}{|l|}{Overall Preference} &
  89 &
  72 &
  39 &
  83 &
  68 &
  50 &
  76 &
  68 &
  56 \\
\multicolumn{1}{|l|}{Game Feel} &
  90 &
  71 &
  40 &
  74 &
  \cellcolor[HTML]{C0C0C0}62 &
  \cellcolor[HTML]{C0C0C0}64 &
  81 &
  62 &
  57 \\
\multicolumn{1}{|l|}{Innovation} &
  \cellcolor[HTML]{C0C0C0}78 &
  \cellcolor[HTML]{C0C0C0}81 &
  42 &
  86 &
  58 &
  51 &
  75 &
  63 &
  62 \\
\multicolumn{1}{|l|}{Thematic Cohesion} &
  78 &
  68 &
  54 &
  93 &
  77 &
  41 &
  91 &
  62 &
  52 \\
\multicolumn{1}{|l|}{Most Interesting Abilities} &
  84 &
  77 &
  39 &
  88 &
  73 &
  39 &
  89 &
  60 &
  51 \\
\multicolumn{1}{|l|}{Visual Presentation} &
  89 &
  69 &
  42 &
  88 &
  \cellcolor[HTML]{C0C0C0}50 &
  \cellcolor[HTML]{C0C0C0}61 &
  77 &
  69 &
  54 \\ \hline
\end{tabular}
\caption{\textbf{Percentage of votes based on the scoring equation $S$ out of their respective maximum possible score for each category and genre.} Models scored with the highest percentage are colored in green, second highest in yellow, and lowest in red.}
\label{tab:score-table}
\end{table*}
